Optimal Transmit Antenna Deployment and Power Allocation for Wireless Power Supply in an Indoor Space

As Internet of Things (IoT) devices proliferate, sustainable methods for powering them are becoming indispensable. The wireless provision of power enables battery-free operation and is crucial for complying with weight and size restrictions. For the energy harvesting (EH) components of these devices to be small, a high operating frequency is necessary. In conjunction with a large transmit antenna, the receivers may be located in the radiating near-field (Fresnel) region, e.g., in indoor scenarios. In this paper, we propose a wireless power transfer (WPT) system ensuring reliable supply of power to an arbitrary number of mobile, low-power, and single-antenna receivers, whose locations in a three-dimensional cuboid room are unknown. A max-min optimisation problem is formulated to determine the optimal transmit power distribution. We rigorously prove that the optimal transmit power distribution's support has a lower dimensionality than its domain and thus, the employment of a continuous aperture antenna, utilised in Holographic MIMO (HMIMO), is unnecessary in the context of the considered WPT problem. Indeed, deploying a discrete transmit antenna architecture, i.e., a transmit antenna array, is sufficient and our proposed solution provides the optimal transmit antenna deployment and power allocation. Moreover, for a one-dimensional transmit antenna architecture, a finite number of transmit antennas is proven to be optimal. The proposed optimal solution is validated through computer simulations. Our simulation results indicate that the optimal transmit antenna architecture requires a finite number of transmit antennas and depends on the geometry of the environment and the dimensionality of the transmit antenna array.

==> Figures/Heatmaps_new/heat.tex <==
% This file was created with tikzplotlib v0.10.1.
\pgfplotsset{every axis title/.append style={at={(0.50,-0.25)}}}
\begin{tikzpicture}[scale=0.95]

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{groupplot}[group style={group size=4 by 2,
    horizontal sep=0.35cm,
    vertical sep=1cm,
    xticklabels at=edge bottom,
    yticklabels at=edge left},
    scale only axis,
    width=3.5cm,
    height=3.5cm]
\nextgroupplot[
tick align=outside,
title={\Large1/1 (2D) (1)},
xmajorticks=false,
x grid style={lightgray204},
xmin=0, xmax=81,
xtick style={color=darkslategray38},
xtick={0.5,11.5,22.5,33.5,44.5,55.5,66.5,77.5},
xticklabels={0,11,22,33,44,55,66,77},
y dir=reverse,
y grid style={lightgray204},
ymajorticks=false,
ymin=0, ymax=81,
yticklabel style={rotate=90.0},
ytick={0.5,10.5,20.5,30.5,40.5,50.5,60.5,70.5,80.5},
yticklabels={0,10,20,30,40,50,60,70,80}
]
\addplot graphics [xmin=0, xmax=81, ymin=81, ymax=0] {Figures/Heatmaps_new/heat-000.png};

\nextgroupplot[
tick align=outside,
title={\Large1/3 (2D) (12)},
xmajorticks=false,
x grid style={lightgray204},
xmin=0, xmax=81,
xtick style={color=darkslategray38},
xtick={0.5,11.5,22.5,33.5,44.5,55.5,66.5,77.5},
xticklabels={0,11,22,33,44,55,66,77},
y dir=reverse,
y grid style={lightgray204},
ymajorticks=false,
ymin=0, ymax=81,
yticklabel style={rotate=90.0},
ytick={0.5,10.5,20.5,30.5,40.5,50.5,60.5,70.5,80.5},
yticklabels={0,10,20,30,40,50,60,70,80}
]
\addplot graphics [xmin=0, xmax=81, ymin=81, ymax=0] {IEEE_OJCOMS-template-LaTex/Figures/Heatmaps_new/heat-001.png};

\nextgroupplot[
tick align=outside,
title={\Large1/4 (2D) (13)},
xmajorticks=false,
xmin=0, xmax=81,
xtick={0.5,11.5,22.5,33.5,44.5,55.5,66.5,77.5},
xticklabels={0,11,22,33,44,55,66,77},
y dir=reverse,
ymajorticks=false,
ymin=0, ymax=81,
ytick={0.5,10.5,20.5,30.5,40.5,50.5,60.5,70.5,80.5},
yticklabels={0,10,20,30,40,50,60,70,80}
]
\addplot graphics [xmin=0, xmax=81, ymin=81, ymax=0] {Figures/Heatmaps_new/heat-002.png};

\nextgroupplot[
tick align=outside,
title={\Large1/5 (2D) (40)},
xmajorticks=false,
xmin=0, xmax=81,
xtick={0.5,11.5,22.5,33.5,44.5,55.5,66.5,77.5},
xticklabels={0,11,22,33,44,55,66,77},
y dir=reverse,
ymajorticks=false,
ymin=0, ymax=81,
ytick={0.5,10.5,20.5,30.5,40.5,50.5,60.5,70.5,80.5},
yticklabels={0,10,20,30,40,50,60,70,80}
]
\addplot graphics [xmin=0, xmax=81, ymin=81, ymax=0] {Figures/Heatmaps_new/heat-003.png};

\nextgroupplot[
tick align=outside,
title={\Large1/1 (1D) (1)},
xmajorticks=false,
xmin=0, xmax=81,
xtick={0.5,11.5,22.5,33.5,44.5,55.5,66.5,77.5},
xticklabels={0,11,22,33,44,55,66,77},
y dir=reverse,
ymajorticks=false,
ymin=0, ymax=81,
ytick={0.5,10.5,20.5,30.5,40.5,50.5,60.5,70.5,80.5},
yticklabels={0,10,20,30,40,50,60,70,80}
]
\addplot graphics [xmin=0, xmax=81, ymin=81, ymax=0] {Figures/Heatmaps_new/heat_new-004.png};

\nextgroupplot[
tick align=outside,
title={\Large1/3 (1D) (4)},
xmajorticks=false,
xmin=0, xmax=81,
xtick={0.5,11.5,22.5,33.5,44.5,55.5,66.5,77.5},
xticklabels={0,11,22,33,44,55,66,77},
y dir=reverse,
ymajorticks=false,
ymin=0, ymax=81,
ytick={0.5,10.5,20.5,30.5,40.5,50.5,60.5,70.5,80.5},
yticklabels={0,10,20,30,40,50,60,70,80}
]
\addplot graphics [xmin=0, xmax=81, ymin=81, ymax=0] {Figures/Heatmaps_new/heat-005.png};

\nextgroupplot[
tick align=outside,
title={\Large1/4 (1D) (4)},
xmajorticks=false,
xmin=0, xmax=81,
xtick={0.5,11.5,22.5,33.5,44.5,55.5,66.5,77.5},
xticklabels={0,11,22,33,44,55,66,77},
y dir=reverse,
ymajorticks=false,
ymin=0, ymax=81,
ytick={0.5,10.5,20.5,30.5,40.5,50.5,60.5,70.5,80.5},
yticklabels={0,10,20,30,40,50,60,70,80}
]
\addplot graphics [xmin=0, xmax=81, ymin=81, ymax=0] {Figures/Heatmaps_new/heat-006.png};

\nextgroupplot[
tick align=outside,
title={\Large1/5 (1D) (4)},
xmajorticks=false,
xmin=0, xmax=81,
xtick={0.5,11.5,22.5,33.5,44.5,55.5,66.5,77.5},
xticklabels={0,11,22,33,44,55,66,77},
y dir=reverse,
ymajorticks=false,
ymin=0, ymax=81,
ytick={0.5,10.5,20.5,30.5,40.5,50.5,60.5,70.5,80.5},
yticklabels={0,10,20,30,40,50,60,70,80}
]
\addplot graphics [xmin=0, xmax=81, ymin=81, ymax=0] {Figures/Heatmaps_new/heat-007.png};
\end{groupplot}


\end{tikzpicture}

